Converge to the Truth: Factual Error Correction via Iterative Constrained Editing

Given a possibly false claim sentence, how can we automatically correct it with minimal editing? Existing methods either require a large number of pairs of false and corrected claims for supervised training or do not handle well errors spanning over multiple tokens within an utterance. In this paper, we propose VENCE, a novel method for factual error correction (FEC) with minimal edits. VENCE formulates the FEC problem as iterative sampling editing actions with respect to a target density function. We carefully design the target function with predicted truthfulness scores from an offline trained fact verification model. VENCE samples the most probable editing positions based on back-calculated gradients of the truthfulness score concerning input tokens and the editing actions using a distantly-supervised language model (T5). Experiments on a public dataset show that VENCE improves the well-adopted SARI metric by 5.3 (or a relative improvement of 11.8%) over the previous best distantly-supervised methods.

==> aaai23bib-backup.tex <==
@inproceedings{ng-etal-2014-conll,
    title = "The {C}o{NLL}-2014 Shared Task on Grammatical Error Correction",
    author = "Ng, Hwee Tou  and
      Wu, Siew Mei  and
      Briscoe, Ted  and
      Hadiwinoto, Christian  and
      Susanto, Raymond Hendy  and
      Bryant, Christopher",
    booktitle = "Proceedings of the Eighteenth Conference on Computational Natural Language Learning: Shared Task",
    month = jun,
    year = "2014",
    address = "Baltimore, Maryland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W14-1701",
    doi = "10.3115/v1/W14-1701",
    pages = "1--14",
}
@article{cobbe2021training,
  title={Training verifiers to solve math word problems},
  author={Cobbe, Karl and Kosaraju, Vineet and Bavarian, Mohammad and Hilton, Jacob and Nakano, Reiichiro and Hesse, Christopher and Schulman, John},
  journal={arXiv preprint arXiv:2110.14168},
  year={2021}
}
@inproceedings{
goyal2022exposing,
title={Exposing the Implicit Energy Networks behind Masked Language Models via Metropolis--Hastings},
author={Kartik Goyal and Chris Dyer and Taylor Berg-Kirkpatrick},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=6PvWo1kEvlT}
}
@inproceedings{bert-score,
  title={BERTScore: Evaluating Text Generation with BERT},
  author={Tianyi Zhang and Varsha Kishore and Felix Wu and Kilian Q. Weinberger and Yoav Artzi},
  booktitle={International Conference on Learning Representations},
  year={2020},
  url={https://openreview.net/forum?id=SkeHuCVFDr}
}
@inproceedings{lin2004rouge,
  title={Rouge: A package for automatic evaluation of summaries},
  author={Lin, Chin-Yew},
  booktitle={Text summarization branches out},
  pages={74--81},
  year={2004}
}
@inproceedings{bryant-etal-2019-bea,
    title = "The {BEA}-2019 Shared Task on Grammatical Error Correction",
    author = "Bryant, Christopher  and
      Felice, Mariano  and
      Andersen, {\O}istein E.  and
      Briscoe, Ted",
    booktitle = "Proceedings of the Fourteenth Workshop on Innovative Use of NLP for Building Educational Applications",
    month = aug,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W19-4406",
    doi = "10.18653/v1/W19-4406",
    pages = "52--75",
}
@inproceedings{aly-etal-2021-fact,
    title = "The Fact Extraction and {VER}ification Over Unstructured and Structured information ({FEVEROUS}) Shared Task",
    author = "Aly, Rami  and
      Guo, Zhijiang  and
      Schlichtkrull, Michael Sejr  and
      Thorne, James  and
      Vlachos, Andreas  and
      Christodoulopoulos, Christos  and
      Cocarascu, Oana  and
      Mittal, Arpit",
    booktitle = "Proceedings of the Fourth Workshop on Fact Extraction and VERification (FEVER)",
    month = nov,
    year = "2021",
    address = "Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.fever-1.1",
    doi = "10.18653/v1/2021.fever-1.1",
    pages = "1--13",
}
@inproceedings{wadden-etal-2020-fact,
    title = "Fact or Fiction: Verifying Scientific Claims",
    author = "Wadden, David  and
      Lin, Shanchuan  and
      Lo, Kyle  and
      Wang, Lucy Lu  and
      van Zuylen, Madeleine  and
      Cohan, Arman  and
      Hajishirzi, Hannaneh",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.609",
    doi = "10.18653/v1/2020.emnlp-main.609",
    pages = "7534--7550",
}
@inproceedings{augenstein-etal-2019-multifc,
    title = "{M}ulti{FC}: A Real-World Multi-Domain Dataset for Evidence-Based Fact Checking of Claims",
    author = "Augenstein, Isabelle  and
      Lioma, Christina  and
      Wang, Dongsheng  and
      Chaves Lima, Lucas  and
      Hansen, Casper  and
      Hansen, Christian  and
      Simonsen, Jakob Grue",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D19-1475",
    doi = "10.18653/v1/D19-1475",
    pages = "4685--4697",
}
@article{Chollampatt_Ng_2018, title={A Multilayer Convolutional Encoder-Decoder Neural Network for Grammatical Error Correction}, volume={32}, url={https://ojs.aaai.org/index.php/AAAI/article/view/12069}, DOI={10.1609/aaai.v32i1.12069}, abstractNote={ &lt;p&gt; We improve automatic correction of grammatical, orthographic, and collocation errors in text using a multilayer convolutional encoder-decoder neural network. The network is initialized with embeddings that make use of character N-gram information to better suit this task. When evaluated on common benchmark test data sets (CoNLL-2014 and JFLEG), our model substantially outperforms all prior neural approaches on this task as well as strong statistical machine translation-based systems with neural and task-specific features trained on the same data. Our analysis shows the superiority of convolutional neural networks over recurrent neural networks such as long short-term memory (LSTM) networks in capturing the local context via attention, and thereby improving the coverage in correcting grammatical errors. By ensembling multiple models, and incorporating an N-gram language model and edit features via rescoring, our novel method becomes the first neural approach to outperform the current state-of-the-art statistical machine translation-based approach, both in terms of grammaticality and fluency. &lt;/p&gt; }, number={1}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Chollampatt, Shamil and Ng, Hwee Tou}, year={2018}, month={Apr.} }
@inproceedings{yuan-briscoe-2016-grammatical,
    title = "Grammatical error correction using neural machine translation",
    author = "Yuan, Zheng  and
      Briscoe, Ted",
    booktitle = "Proceedings of the 2016 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies",
    month = jun,
    year = "2016",
    address = "San Diego, California",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/N16-1042",
    doi = "10.18653/v1/N16-1042",
    pages = "380--386",
}
@inproceedings{yasunaga-etal-2021-lm,
    title = "{LM}-Critic: Language Models for Unsupervised Grammatical Error Correction",
    author = "Yasunaga, Michihiro  and
      Leskovec, Jure  and
      Liang, Percy",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.611",
    doi = "10.18653/v1/2021.emnlp-main.611",
    pages = "7752--7763",
    abstract = "Grammatical error correction (GEC) requires a set of labeled ungrammatical / grammatical sentence pairs for training, but obtaining such annotation can be prohibitively expensive. Recently, the Break-It-Fix-It (BIFI) framework has demonstrated strong results on learning to repair a broken program without any labeled examples, but this relies on a perfect critic (e.g., a compiler) that returns whether an example is valid or not, which does not exist for the GEC task. In this work, we show how to leverage a pretrained language model (LM) in defining an LM-Critic, which judges a sentence to be grammatical if the LM assigns it a higher probability than its local perturbations. We apply this LM-Critic and BIFI along with a large set of unlabeled sentences to bootstrap realistic ungrammatical / grammatical pairs for training a corrector. We evaluate our approach on GEC datasets on multiple domains (CoNLL-2014, BEA-2019, GMEG-wiki and GMEG-yahoo) and show that it outperforms existing methods in both the unsupervised setting (+7.7 F0.5) and the supervised setting (+0.5 F0.5).",
}
@article{krishna-riedel-vlachos-2021-proofver,
  author    = {Amrith Krishna and
               Sebastian Riedel and
               Andreas Vlachos},
  title     = {ProoFVer: Natural Logic Theorem Proving for Fact Verification},
  journal   = {CoRR},
  volume    = {abs/2108.11357},
  year      = {2021},
  url       = {https://arxiv.org/abs/2108.11357},
  eprinttype = {arXiv},
  eprint    = {2108.11357},
  timestamp = {Fri, 27 Aug 2021 15:02:29 +0200},
}

@inproceedings{thorne-etal-2018-fever,
    title = "{FEVER}: a Large-scale Dataset for Fact Extraction and {VER}ification",
    author = "Thorne, James  and
      Vlachos, Andreas  and
      Christodoulopoulos, Christos  and
      Mittal, Arpit",
    booktitle = "Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)",
    month = jun,
    year = "2018",
    address = "New Orleans, Louisiana",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/N18-1074",
    doi = "10.18653/v1/N18-1074",
    pages = "809--819",
}
@article{Chen_Bao_Sun_Zhang_Chen_Zhou_Xiao_Li_2022, title={LOREN: Logic-Regularized Reasoning for Interpretable Fact Verification}, volume={36}, url={https://ojs.aaai.org/index.php/AAAI/article/view/21291}, DOI={10.1609/aaai.v36i10.21291}, abstractNote={Given a natural language statement, how to verify its veracity against a large-scale textual knowledge source like Wikipedia? Most existing neural models make predictions without giving clues about which part of a false claim goes wrong. In this paper, we propose LOREN, an approach for interpretable fact verification. We decompose the verification of the whole claim at phrase-level, where the veracity of the phrases serves as explanations and can be aggregated into the final verdict according to logical rules. The key insight of LOREN is to represent claim phrase veracity as three-valued latent variables, which are regularized by aggregation logical rules. The final claim verification is based on all latent variables. Thus, LOREN enjoys the additional benefit of interpretability --- it is easy to explain how it reaches certain results with claim phrase veracity. Experiments on a public fact verification benchmark show that LOREN is competitive against previous approaches while enjoying the merit of faithful and accurate interpretability. The resources of LOREN are available at: https://github.com/jiangjiechen/LOREN.}, number={10}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Chen, Jiangjie and Bao, Qiaoben and Sun, Changzhi and Zhang, Xinbo and Chen, Jiaze and Zhou, Hao and Xiao, Yanghua and Li, Lei}, year={2022}, month={Jun.}, pages={10482-10491} }
@inproceedings{hayate-qiao-li-2020-fact,
	doi = {10.18653/v1/2020.acl-main.17},
	url = {https://doi.org/10.18653%2Fv1%2F2020.acl-main.17},
	year = 2020,
	publisher = {Association for Computational Linguistics},
	author = {Hayate Iso and Chao Qiao and Hang Li},
	title = {Fact-based Text Editing},
	booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics}
}
@inproceedings{inui-etal-2003-text,
    title = "Text Simplification for Reading Assistance: A Project Note",
    author = "Inui, Kentaro  and
      Fujita, Atsushi  and
      Takahashi, Tetsuro  and
      Iida, Ryu  and
      Iwakura, Tomoya",
    booktitle = "Proceedings of the Second International Workshop on Paraphrasing",
    month = jul,
    year = "2003",
    address = "Sapporo, Japan",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W03-1602",
    doi = "10.3115/1118984.1118986",
    pages = "9--16",
}
@article{hu-etal-2022-text,
  title={Text style transfer: A review and experimental evaluation},
  author={Hu, Zhiqiang and Lee, Roy Ka-Wei and Aggarwal, Charu C and Zhang, Aston},
  journal={ACM SIGKDD Explorations Newsletter},
  volume={24},
  number={1},
  pages={14--45},
  year={2022},
  publisher={ACM New York, NY, USA}
}
@inproceedings{omelianchuk-etal-2020-gector,
    title = "{GECT}o{R} {--} Grammatical Error Correction: Tag, Not Rewrite",
    author = "Omelianchuk, Kostiantyn  and
      Atrasevych, Vitaliy  and
      Chernodub, Artem  and
      Skurzhanskyi, Oleksandr",
    booktitle = "Proceedings of the Fifteenth Workshop on Innovative Use of NLP for Building Educational Applications",
    month = jul,
    year = "2020",
    address = "Seattle, WA, USA → Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.bea-1.16",
    doi = "10.18653/v1/2020.bea-1.16",
    pages = "163--170",
}
@article{hinton2002training,
  title={Training products of experts by minimizing contrastive divergence},
  author={Hinton, Geoffrey E},
  journal={Neural computation},
  volume={14},
  number={8},
  pages={1771--1800},
  year={2002},
  publisher={MIT Press}
}
@article{metropolis1953equation,
  title={Equation of state calculations by fast computing machines},
  author={Metropolis, Nicholas and Rosenbluth, Arianna W and Rosenbluth, Marshall N and Teller, Augusta H and Teller, Edward},
  journal={The journal of chemical physics},
  volume={21},
  number={6},
  pages={1087--1092},
  year={1953},
  publisher={American Institute of Physics}
}
@inproceedings{lewis-etal-2020-bart,
    title = "{BART}: Denoising Sequence-to-Sequence Pre-training for Natural Language Generation, Translation, and Comprehension",
    author = "Lewis, Mike  and
      Liu, Yinhan  and
      Goyal, Naman  and
      Ghazvininejad, Marjan  and
      Mohamed, Abdelrahman  and
      Levy, Omer  and
      Stoyanov, Veselin  and
      Zettlemoyer, Luke",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/2020.acl-main.703",
    doi = "10.18653/v1/2020.acl-main.703",
    pages = "7871--7880",
}
@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/N19-1423",
    doi = "10.18653/v1/N19-1423",
    pages = "4171--4186",
}
@article{xu-etal-2016-optimizing,
    title = "Optimizing Statistical Machine Translation for Text Simplification",
    author = "Xu, Wei  and
      Napoles, Courtney  and
      Pavlick, Ellie  and
      Chen, Quanze  and
      Callison-Burch, Chris",
    journal = "Transactions of the Association for Computational Linguistics",
    volume = "4",
    year = "2016",
    address = "Cambridge, MA",
    publisher = "MIT Press",
    url = "https://aclanthology.org/Q16-1029",
    doi = "10.1162/tacl_a_00107",
    pages = "401--415",
}
@article{Miao_Zhou_Mou_Yan_Li_2019, 
    title={CGMH: Constrained Sentence Generation by Metropolis-Hastings Sampling}, 
    volume={33}, 
    url={https://ojs.aaai.org/index.php/AAAI/article/view/4659}, 
    DOI={10.1609/aaai.v33i01.33016834}, 
    abstractNote={&lt;p&gt;In real-world applications of natural language generation, 
    there are often constraints on the target sentences in addition to fluency and naturalness requirements. Existing language generation techniques are usually based on recurrent neural networks (RNNs). However, it is non-trivial to impose constraints on RNNs while maintaining generation quality, since RNNs generate sentences sequentially (or with beam search) from the first word to the last. In this paper, we propose CGMH, a novel approach using Metropolis-Hastings sampling for constrained sentence generation. CGMH allows complicated constraints such as the occurrence of multiple keywords in the target sentences, which cannot be handled in traditional RNN-based approaches. Moreover, CGMH works in the inference stage, and does not require parallel corpora for training. We evaluate our method on a variety of tasks, including keywords-to-sentence generation, unsupervised sentence paraphrasing, and unsupervised sentence error correction. CGMH achieves high performance compared with previous supervised methods for sentence generation. Our code is released at https://github.com/NingMiao/CGMH&lt;/p&gt;}, 
    number={01}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Miao, Ning and Zhou, Hao and Mou, Lili and Yan, Rui and Li, Lei}, 
    year={2019}, 
    month={Jul.}, 
    pages={6834-6842} 
}
@article{mallinson2022edit5,
  title={EdiT5: Semi-Autoregressive Text-Editing with T5 Warm-Start},
  author={Mallinson, Jonathan and Adamek, Jakub and Malmi, Eric and Severyn, Aliaksei},
  journal={arXiv preprint arXiv:2205.12209},
  year={2022}
}
@inproceedings{karpukhin-etal-2020-dense,
    title = "Dense Passage Retrieval for Open-Domain Question Answering",
    author = "Karpukhin, Vladimir  and
      Oguz, Barlas  and
      Min, Sewon  and
      Lewis, Patrick  and
      Wu, Ledell  and
      Edunov, Sergey  and
      Chen, Danqi  and
      Yih, Wen-tau",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.550",
    doi = "10.18653/v1/2020.emnlp-main.550",
    pages = "6769--6781",
}
@inproceedings{
cao2021autoregressive,
title={Autoregressive Entity Retrieval},
author={Nicola De Cao and Gautier Izacard and Sebastian Riedel and Fabio Petroni},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=5k8F6UU39V}
}
@article{Shah_Schuster_Barzilay_2020, 
    title={Automatic Fact-Guided Sentence Modification}, 
    volume={34}, 
    url={https://ojs.aaai.org/index.php/AAAI/article/view/6406}, 
    DOI={10.1609/aaai.v34i05.6406}, 
    abstractNote={&lt;p&gt;Online encyclopediae like Wikipedia contain large amounts of text that need frequent corrections and updates. The new information may contradict existing content in encyclopediae. In this paper, we focus on rewriting such dynamically changing articles. This is a challenging constrained generation task, as the output must be consistent with the new information and fit into the rest of the existing document. To this end, we propose a two-step solution: (1) We identify and remove the contradicting components in a target text for a given claim, using a neutralizing stance model; (2) We expand the remaining text to be consistent with the given claim, using a novel two-encoder sequence-to-sequence model with copy attention. Applied to a Wikipedia fact update dataset, our method successfully generates updated sentences for new claims, achieving the highest SARI score. Furthermore, we demonstrate that generating synthetic data through such rewritten sentences can successfully augment the FEVER fact-checking training dataset, leading to a relative error reduction of 13%.&lt;sup&gt;1&lt;/sup&gt;&lt;/p&gt;}, 
    number={05}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Shah, Darsh and Schuster, Tal and Barzilay, Regina}, 
    year={2020}, 
    month={Apr.}, 
    pages={8791-8798} 
}
@inproceedings{sha-2020-gradient,
    title = "Gradient-guided Unsupervised Lexically Constrained Text Generation",
    author = "Sha, Lei",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.701",
    doi = "10.18653/v1/2020.emnlp-main.701",
    pages = "8692--8703",
}
@article{ji2022survey,
  title={Survey of hallucination in natural language generation},
  author={Ji, Ziwei and Lee, Nayeon and Frieske, Rita and Yu, Tiezheng and Su, Dan and Xu, Yan and Ishii, Etsuko and Bang, Yejin and Madotto, Andrea and Fung, Pascale},
  journal={arXiv preprint arXiv:2202.03629},
  year={2022}
}
@inproceedings{iv-etal-2022-fruit,
    title = "{FRUIT}: Faithfully Reflecting Updated Information in Text",
    author = "Iv, Robert  and
      Passos, Alexandre  and
      Singh, Sameer  and
      Chang, Ming-Wei",
    booktitle = "Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies",
    month = jul,
    year = "2022",
    address = "Seattle, United States",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.naacl-main.269",
    doi = "10.18653/v1/2022.naacl-main.269",
    pages = "3670--3686",
    abstract = "Textual knowledge bases such as Wikipedia require considerable effort to keep up to date and consistent. While automated writing assistants could potentially ease this burden, the problem of suggesting edits grounded in external knowledge has been under-explored. In this paper, we introduce the novel generation task of *faithfully reflecting updated information in text* (FRUIT) where the goal is to update an existing article given new evidence. We release the FRUIT-WIKI dataset, a collection of over 170K distantly supervised data produced from pairs of Wikipedia snapshots, along with our data generation pipeline and a gold evaluation set of 914 instances whose edits are guaranteed to be supported by the evidence. We provide benchmark results for popular generation systems as well as EDIT5 {--} a T5-based approach tailored to editing we introduce that establishes the state of the art. Our analysis shows that developing models that can update articles faithfully requires new capabilities for neural generation models, and opens doors to many new applications.",
}
@inproceedings{gardent-etal-2017-creating,
    title = "Creating Training Corpora for {NLG} Micro-Planners",
    author = "Gardent, Claire  and
      Shimorina, Anastasia  and
      Narayan, Shashi  and
      Perez-Beltrachini, Laura",
    booktitle = "Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P17-1017",
    doi = "10.18653/v1/P17-1017",
    pages = "179--188",
    abstract = "In this paper, we present a novel framework for semi-automatically creating linguistically challenging micro-planning data-to-text corpora from existing Knowledge Bases. Because our method pairs data of varying size and shape with texts ranging from simple clauses to short texts, a dataset created using this framework provides a challenging benchmark for microplanning. Another feature of this framework is that it can be applied to any large scale knowledge base and can therefore be used to train and learn KB verbalisers. We apply our framework to DBpedia data and compare the resulting dataset with Wen et al. 2016{'}s. We show that while Wen et al.{'}s dataset is more than twice larger than ours, it is less diverse both in terms of input and in terms of text. We thus propose our corpus generation framework as a novel method for creating challenging data sets from which NLG models can be learned which are capable of handling the complex interactions occurring during in micro-planning between lexicalisation, aggregation, surface realisation, referring expression generation and sentence segmentation. To encourage researchers to take up this challenge, we made available a dataset of 21,855 data/text pairs created using this framework in the context of the WebNLG shared task.",
}
@inproceedings{chen-etal-2021-improving,
    title = "Improving Faithfulness in Abstractive Summarization with Contrast Candidate Generation and Selection",
    author = "Chen, Sihao  and
      Zhang, Fan  and
      Sone, Kazoo  and
      Roth, Dan",
    booktitle = "Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies",
    month = jun,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.naacl-main.475",
    doi = "10.18653/v1/2021.naacl-main.475",
    pages = "5935--5941",
    abstract = "Despite significant progress in neural abstractive summarization, recent studies have shown that the current models are prone to generating summaries that are unfaithful to the original context. To address the issue, we study contrast candidate generation and selection as a model-agnostic post-processing technique to correct the extrinsic hallucinations (i.e. information not present in the source text) in unfaithful summaries. We learn a discriminative correction model by generating alternative candidate summaries where named entities and quantities in the generated summary are replaced with ones with compatible semantic types from the source document. This model is then used to select the best candidate as the final output summary. Our experiments and analysis across a number of neural summarization systems show that our proposed method is effective in identifying and correcting extrinsic hallucinations. We analyze the typical hallucination phenomenon by different types of neural summarization systems, in hope to provide insights for future work on the direction.",
}
@inproceedings{xu-etal-2021-agggen,
    title = "{A}gg{G}en: Ordering and Aggregating while Generating",
    author = "Xu, Xinnuo  and
      Du{\v{s}}ek, Ond{\v{r}}ej  and
      Rieser, Verena  and
      Konstas, Ioannis",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.acl-long.113",
    doi = "10.18653/v1/2021.acl-long.113",
    pages = "1419--1434",
    abstract = "We present AggGen (pronounced {`}again{'}) a data-to-text model which re-introduces two explicit sentence planning stages into neural data-to-text systems: input ordering and input aggregation. In contrast to previous work using sentence planning, our model is still end-to-end: AggGen performs sentence planning at the same time as generating text by learning latent alignments (via semantic facts) between input representation and target text. Experiments on the WebNLG and E2E challenge data show that by using fact-based alignments our approach is more interpretable, expressive, robust to noise, and easier to control, while retaining the advantages of end-to-end systems in terms of fluency. Our code is available at https://github.com/XinnuoXu/AggGen.",
}
@inproceedings{thorne-vlachos-2021-evidence,
    title = "Evidence-based Factual Error Correction",
    author = "Thorne, James  and
      Vlachos, Andreas",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.acl-long.256",
    doi = "10.18653/v1/2021.acl-long.256",
    pages = "3298--3309",
    abstract = "This paper introduces the task of factual error correction: performing edits to a claim so that the generated rewrite is better supported by evidence. This extends the well-studied task of fact verification by providing a mechanism to correct written texts that are refuted or only partially supported by evidence. We demonstrate that it is feasible to train factual error correction systems from existing fact checking datasets which only contain labeled claims accompanied by evidence, but not the correction. We achieve this by employing a two-stage distant supervision approach that incorporates evidence into masked claims when generating corrections. Our approach, based on the T5 transformer and using retrieved evidence, achieved better results than existing work which used a pointer copy network and gold evidence, producing accurate factual error corrections for 5x more instances in human evaluation and a .125 increase in SARI score. The evaluation is conducted on a dataset of 65,000 instances based on a recent fact verification shared task and we release it to enable further work on the task.",
}
@article{raffel-etal-2020-exploring,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer.},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J and others},
  journal={J. Mach. Learn. Res.},
  volume={21},
  number={140},
  pages={1--67},
  year={2020}
}
@article{radford2019language,
  title={Language models are unsupervised multitask learners},
  author={Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
  journal={OpenAI Blog},
  volume={1},
  number={8},
  pages={9},
  year={2019}
}
@inproceedings{NEURIPS2020_1457c0d6,
 author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel and Wu, Jeffrey and Winter, Clemens and Hesse, Chris and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Larochelle and M. Ranzato and R. Hadsell and M.F. Balcan and H. Lin},
 pages = {1877--1901},
 publisher = {Curran Associates, Inc.},
 title = {Language Models are Few-Shot Learners},
 url = {https://proceedings.neurips.cc/paper/2020/file/1457c0d6bfcb4967418bfb8ac142f64a-Paper.pdf},
 volume = {33},
 year = {2020}
}
@inproceedings{mireshghallah-etal-2022-mix,
    title = "Mix and Match: Learning-free Controllable Text Generationusing Energy Language Models",
    author = "Mireshghallah, Fatemehsadat  and
      Goyal, Kartik  and
      Berg-Kirkpatrick, Taylor",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.31",
    doi = "10.18653/v1/2022.acl-long.31",
    pages = "401--415",
    abstract = "Recent work on controlled text generation has either required attribute-based fine-tuning of the base language model (LM), or has restricted the parameterization of the attribute discriminator to be compatible with the base autoregressive LM. In this work, we propose Mix and Match LM, a global score-based alternative for controllable text generation that combines arbitrary pre-trained black-box models for achieving the desired attributes in the generated text without involving any fine-tuning or structural assumptions about the black-box models. We interpret the task of controllable generation as drawing samples from an energy-based model whose energy values are a linear combination of scores from black-box models that are separately responsible for fluency, the control attribute, and faithfulness to any conditioning context. We use a Metropolis-Hastings sampling scheme to sample from this energy-based model using bidirectional context and global attribute features. We validate the effectiveness of our approach on various controlled generation and style-based text revision tasks by outperforming recently proposed methods that involve extra training, fine-tuning, or restrictive assumptions over the form of models.",
}
@inproceedings{lee-etal-2020-noising,
    title = "Noising Scheme for Data Augmentation in Automatic Post-Editing",
    author = "Lee, WonKee  and
      Shin, Jaehun  and
      Jung, Baikjin  and
      Lee, Jihyung  and
      Lee, Jong-Hyeok",
    booktitle = "Proceedings of the Fifth Conference on Machine Translation",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.wmt-1.83",
    pages = "783--788",
}
@inproceedings{Nie2019CombiningFE,
  title={Combining Fact Extraction and Verification with Neural Semantic Matching Networks},
  author={Yixin Nie and H. Chen and Mohit Bansal},
  booktitle={AAAI},
  year={2019}
}
@inproceedings{wu-etal-2021-unified,
    title = "Unified Dual-view Cognitive Model for Interpretable Claim Verification",
    author = "Wu, Lianwei  and
      Rao, Yuan  and
      Lan, Yuqian  and
      Sun, Ling  and
      Qi, Zhaoyin",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.acl-long.5",
    doi = "10.18653/v1/2021.acl-long.5",
    pages = "59--68",
    abstract = "Recent studies constructing direct interactions between the claim and each single user response (a comment or a relevant article) to capture evidence have shown remarkable success in interpretable claim verification. Owing to different single responses convey different cognition of individual users (i.e., audiences), the captured evidence belongs to the perspective of individual cognition. However, individuals{'} cognition of social things is not always able to truly reflect the objective. There may be one-sided or biased semantics in their opinions on a claim. The captured evidence correspondingly contains some unobjective and biased evidence fragments, deteriorating task performance. In this paper, we propose a Dual-view model based on the views of Collective and Individual Cognition (CICD) for interpretable claim verification. From the view of the collective cognition, we not only capture the word-level semantics based on individual users, but also focus on sentence-level semantics (i.e., the overall responses) among all users and adjust the proportion between them to generate global evidence. From the view of individual cognition, we select the top-$k$ articles with high degree of difference and interact with the claim to explore the local key evidence fragments. To weaken the bias of individual cognition-view evidence, we devise inconsistent loss to suppress the divergence between global and local evidence for strengthening the consistent shared evidence between the both. Experiments on three benchmark datasets confirm that CICD achieves state-of-the-art performance.",
}
@inproceedings{kotonya-etal-2021-graph,
    title = "Graph Reasoning with Context-Aware Linearization for Interpretable Fact Extraction and Verification",
    author = "Kotonya, Neema  and
      Spooner, Thomas  and
      Magazzeni, Daniele  and
      Toni, Francesca",
    booktitle = "Proceedings of the Fourth Workshop on Fact Extraction and VERification (FEVER)",
    month = nov,
    year = "2021",
    address = "Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.fever-1.3",
    doi = "10.18653/v1/2021.fever-1.3",
    pages = "21--30",
    abstract = "This paper presents an end-to-end system for fact extraction and verification using textual and tabular evidence, the performance of which we demonstrate on the FEVEROUS dataset. We experiment with both a multi-task learning paradigm to jointly train a graph attention network for both the task of evidence extraction and veracity prediction, as well as a single objective graph model for solely learning veracity prediction and separate evidence extraction. In both instances, we employ a framework for per-cell linearization of tabular evidence, thus allowing us to treat evidence from tables as sequences. The templates we employ for linearizing tables capture the context as well as the content of table data. We furthermore provide a case study to show the interpretability our approach. Our best performing system achieves a FEVEROUS score of 0.23 and 53{\%} label accuracy on the blind test data.",
}
@inproceedings{maynez-etal-2020-faithfulness,
    title = "On Faithfulness and Factuality in Abstractive Summarization",
    author = "Maynez, Joshua  and
      Narayan, Shashi  and
      Bohnet, Bernd  and
      McDonald, Ryan",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.acl-main.173",
    doi = "10.18653/v1/2020.acl-main.173",
    pages = "1906--1919",
    abstract = "It is well known that the standard likelihood training and approximate decoding objectives in neural text generation models lead to less human-like responses for open-ended tasks such as language modeling and story generation. In this paper we have analyzed limitations of these models for abstractive document summarization and found that these models are highly prone to hallucinate content that is unfaithful to the input document. We conducted a large scale human evaluation of several neural abstractive summarization systems to better understand the types of hallucinations they produce. Our human annotators found substantial amounts of hallucinated content in all model generated summaries. However, our analysis does show that pretrained models are better summarizers not only in terms of raw metrics, i.e., ROUGE, but also in generating faithful and factual summaries as evaluated by humans. Furthermore, we show that textual entailment measures better correlate with faithfulness than standard metrics, potentially leading the way to automatic evaluation metrics as well as training and decoding criteria.",
}
@inproceedings{raunak-etal-2021-curious,
    title = "The Curious Case of Hallucinations in Neural Machine Translation",
    author = "Raunak, Vikas  and
      Menezes, Arul  and
      Junczys-Dowmunt, Marcin",
    booktitle = "Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies",
    month = jun,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.naacl-main.92",
    doi = "10.18653/v1/2021.naacl-main.92",
    pages = "1172--1183",
    abstract = "In this work, we study hallucinations in Neural Machine Translation (NMT), which lie at an extreme end on the spectrum of NMT pathologies. Firstly, we connect the phenomenon of hallucinations under source perturbation to the Long-Tail theory of Feldman, and present an empirically validated hypothesis that explains hallucinations under source perturbation. Secondly, we consider hallucinations under corpus-level noise (without any source perturbation) and demonstrate that two prominent types of natural hallucinations (detached and oscillatory outputs) could be generated and explained through specific corpus-level noise patterns. Finally, we elucidate the phenomenon of hallucination amplification in popular data-generation processes such as Backtranslation and sequence-level Knowledge Distillation. We have released the datasets and code to replicate our results.",
}
@inproceedings{stammbach2020fever,
  title={e-fever: Explanations and summaries for automated fact checking},
  author={Stammbach, Dominik and Ash, Elliott},
  booktitle={Proceedings of the 2020 Truth and Trust Online Conference (TTO 2020)},
  pages={32},
  year={2020},
  organization={Hacks Hackers}
}
@inproceedings{samarinas-etal-2021-improving,
    title = "Improving Evidence Retrieval for Automated Explainable Fact-Checking",
    author = "Samarinas, Chris  and
      Hsu, Wynne  and
      Lee, Mong Li",
    booktitle = "Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies: Demonstrations",
    month = jun,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.naacl-demos.10",
    doi = "10.18653/v1/2021.naacl-demos.10",
    pages = "84--91",
    abstract = "Automated fact-checking on a large-scale is a challenging task that has not been studied systematically until recently. Large noisy document collections like the web or news articles make the task more difficult. We describe a three-stage automated fact-checking system, named Quin+, using evidence retrieval and selection methods. We demonstrate that using dense passage representations leads to much higher evidence recall in a noisy setting. We also propose two sentence selection approaches, an embedding-based selection using a dense retrieval model, and a sequence labeling approach for context-aware selection. Quin+ is able to verify open-domain claims using results from web search engines.",
}
@inproceedings{agrawal-carpuat-2022-imitation,
    title = "An Imitation Learning Curriculum for Text Editing with Non-Autoregressive Models",
    author = "Agrawal, Sweta  and
      Carpuat, Marine",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.520",
    doi = "10.18653/v1/2022.acl-long.520",
    pages = "7550--7563",
}
@inproceedings{kasner-dusek-2020-data,
    title = "Data-to-Text Generation with Iterative Text Editing",
    author = "Kasner, Zden{\v{e}}k  and
      Du{\v{s}}ek, Ond{\v{r}}ej",
    booktitle = "Proceedings of the 13th International Conference on Natural Language Generation",
    month = dec,
    year = "2020",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.inlg-1.9",
    pages = "60--67",
}
@inproceedings{higashiyama-etal-2021-text,
    title = "A Text Editing Approach to Joint {J}apanese Word Segmentation, {POS} Tagging, and Lexical Normalization",
    author = "Higashiyama, Shohei  and
      Utiyama, Masao  and
      Watanabe, Taro  and
      Sumita, Eiichiro",
    booktitle = "Proceedings of the Seventh Workshop on Noisy User-generated Text (W-NUT 2021)",
    month = nov,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.wnut-1.9",
    doi = "10.18653/v1/2021.wnut-1.9",
    pages = "67--80",
}
@article{Chen_Gan_Cheng_Zhou_Xiao_Li_2022,
  title        = {Unsupervised Editing for Counterfactual Stories},
  volume       = {36},
  url          = {https://ojs.aaai.org/index.php/AAAI/article/view/21290},
  doi          = {10.1609/aaai.v36i10.21290},
  abstractnote = {Creating what-if stories requires reasoning about prior statements and possible outcomes of the changed conditions. One can easily generate coherent endings under new conditions, but it would be challenging for current systems to do it with minimal changes to the original story. Therefore, one major challenge is the trade-off between generating a logical story and rewriting with minimal-edits. In this paper, we propose EDUCAT, an editing-based unsupervised approach for counterfactual story rewriting. EDUCAT includes a target position detection strategy based on estimating causal effects of the what-if conditions, which keeps the causal invariant parts of the story. EDUCAT then generates the stories under fluency, coherence and minimal-edits constraints. We also propose a new metric to alleviate the shortcomings of current automatic metrics and better evaluate the trade-off. We evaluate EDUCAT on a public counterfactual story rewriting benchmark. Experiments show that EDUCAT achieves the best trade-off over unsupervised SOTA methods according to both automatic and human evaluation. The resources of EDUCAT are available at: https://github.com/jiangjiechen/EDUCAT.},
  number       = {10},
  journal      = {Proceedings of the AAAI Conference on Artificial Intelligence},
  author       = {Chen, Jiangjie and Gan, Chun and Cheng, Sijie and Zhou, Hao and Xiao, Yanghua and Li, Lei},
  year         = {2022},
  month        = {Jun.},
  pages        = {10473-10481}
}
@inproceedings{kotonya-toni-2020-explainable,
    title = "Explainable Automated Fact-Checking: A Survey",
    author = "Kotonya, Neema  and
      Toni, Francesca",
    booktitle = "Proceedings of the 28th International Conference on Computational Linguistics",
    month = dec,
    year = "2020",
    address = "Barcelona, Spain (Online)",
    publisher = "International Committee on Computational Linguistics",
    url = "https://aclanthology.org/2020.coling-main.474",
    doi = "10.18653/v1/2020.coling-main.474",
    pages = "5430--5443",
    abstract = "A number of exciting advances have been made in automated fact-checking thanks to increasingly larger datasets and more powerful systems, leading to improvements in the complexity of claims which can be accurately fact-checked. However, despite these advances, there are still desirable functionalities missing from the fact-checking pipeline. In this survey, we focus on the explanation functionality {--} that is fact-checking systems providing reasons for their predictions. We summarize existing methods for explaining the predictions of fact-checking systems and we explore trends in this topic. Further, we consider what makes for good explanations in this specific domain through a comparative analysis of existing fact-checking explanations against some desirable properties. Finally, we propose further research directions for generating fact-checking explanations, and describe how these may lead to improvements in the research area.",
}
@inproceedings{cao-etal-2022-hallucinated,
    title = "Hallucinated but Factual! Inspecting the Factuality of Hallucinations in Abstractive Summarization",
    author = "Cao, Meng  and
      Dong, Yue  and
      Cheung, Jackie",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.236",
    doi = "10.18653/v1/2022.acl-long.236",
    pages = "3340--3354",
}
@article{Cao_Wei_Li_Li_2018, title={Faithful to the Original: Fact Aware Neural Abstractive Summarization}, volume={32}, url={https://ojs.aaai.org/index.php/AAAI/article/view/11912}, DOI={10.1609/aaai.v32i1.11912}, number={1}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Cao, Ziqiang and Wei, Furu and Li, Wenjie and Li, Sujian}, year={2018}, month={Apr.} }
@inproceedings{NEURIPS2019_675f9820,
 author = {Gu, Jiatao and Wang, Changhan and Zhao, Junbo},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Levenshtein Transformer},
 url = {https://proceedings.neurips.cc/paper/2019/file/675f9820626f5bc0afb47b57890b466e-Paper.pdf},
 volume = {32},
 year = {2019}
}
@inproceedings{zhang-etal-2020-language-generation,
    title = "Language Generation via Combinatorial Constraint Satisfaction: A Tree Search Enhanced {M}onte-{C}arlo Approach",
    author = "Zhang, Maosen  and
      Jiang, Nan  and
      Li, Lei  and
      Xue, Yexiang",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2020",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.findings-emnlp.115",
    doi = "10.18653/v1/2020.findings-emnlp.115",
    pages = "1286--1298",
    abstract = "Generating natural language under complex constraints is a principled formulation towards controllable text generation. We present a framework to allow specification of combinatorial constraints for sentence generation. We propose TSMC, an efficient method to generate high likelihood sentences with respect to a pre-trained language model while satisfying the constraints. Our approach is highly flexible, requires no task-specific train- ing, and leverages efficient constraint satisfaction solving techniques. To better handle the combinatorial constraints, a tree search algorithm is embedded into the proposal process of the Markov Chain Monte Carlo (MCMC) to explore candidates that satisfy more constraints. Compared to existing MCMC approaches, our sampling approach has a better mixing performance. Experiments show that TSMC achieves consistent and significant improvement on multiple language generation tasks.",
}
@inproceedings{qorib-etal-2022-frustratingly,
    title = "Frustratingly Easy System Combination for Grammatical Error Correction",
    author = "Qorib, Muhammad  and
      Na, Seung-Hoon  and
      Ng, Hwee Tou",
    booktitle = "Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies",
    month = jul,
    year = "2022",
    address = "Seattle, United States",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.naacl-main.143",
    pages = "1964--1974",
}
@inproceedings{ishii-etal-2021-grammatical,
    title = "Grammatical Error Correction via Supervised Attention in the Vicinity of Errors",
    author = "Ishii, Hiromichi  and
      Tamura, Akihiro  and
      Ninomiya, Takashi",
    booktitle = "Proceedings of the 35th Pacific Asia Conference on Language, Information and Computation",
    month = "11",
    year = "2021",
    address = "Shanghai, China",
    publisher = "Association for Computational Lingustics",
    url = "https://aclanthology.org/2021.paclic-1.24",
    pages = "227--234",
}
@inproceedings{parnow-etal-2021-grammatical,
    title = "Grammatical Error Correction as {GAN}-like Sequence Labeling",
    author = "Parnow, Kevin  and
      Li, Zuchao  and
      Zhao, Hai",
    booktitle = "Findings of the Association for Computational Linguistics: ACL-IJCNLP 2021",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.findings-acl.290",
    doi = "10.18653/v1/2021.findings-acl.290",
    pages = "3284--3290",
}
@inproceedings{williams-etal-2018-broad,
    title = "A Broad-Coverage Challenge Corpus for Sentence Understanding through Inference",
    author = "Williams, Adina  and
      Nangia, Nikita  and
      Bowman, Samuel",
    booktitle = "Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)",
    month = jun,
    year = "2018",
    address = "New Orleans, Louisiana",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/N18-1101",
    doi = "10.18653/v1/N18-1101",
    pages = "1112--1122",
}
@article{liu2019roberta,
  title={Roberta: A robustly optimized bert pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}
@inproceedings{xiao-wang-2021-hallucination,
    title = "On Hallucination and Predictive Uncertainty in Conditional Language Generation",
    author = "Xiao, Yijun  and
      Wang, William Yang",
    booktitle = "Proceedings of the 16th Conference of the European Chapter of the Association for Computational Linguistics: Main Volume",
    month = apr,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.eacl-main.236",
    doi = "10.18653/v1/2021.eacl-main.236",
    pages = "2734--2744",
}
@inproceedings{ladhak-etal-2022-faithful,
    title = "Faithful or Extractive? On Mitigating the Faithfulness-Abstractiveness Trade-off in Abstractive Summarization",
    author = "Ladhak, Faisal  and
      Durmus, Esin  and
      He, He  and
      Cardie, Claire  and
      McKeown, Kathleen",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.100",
    doi = "10.18653/v1/2022.acl-long.100",
    pages = "1410--1421",
}
@inproceedings{devaraj-etal-2022-evaluating,
    title = "Evaluating Factuality in Text Simplification",
    author = "Devaraj, Ashwin  and
      Sheffield, William  and
      Wallace, Byron  and
      Li, Junyi Jessy",
    booktitle = "Proceedings of the 60th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = may,
    year = "2022",
    address = "Dublin, Ireland",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.acl-long.506",
    doi = "10.18653/v1/2022.acl-long.506",
    pages = "7331--7345",
}
@inproceedings{honovich-etal-2021-q2,
    title = "$Q^{2}$: {E}valuating Factual Consistency in Knowledge-Grounded Dialogues via Question Generation and Question Answering",
    author = "Honovich, Or  and
      Choshen, Leshem  and
      Aharoni, Roee  and
      Neeman, Ella  and
      Szpektor, Idan  and
      Abend, Omri",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.619",
    doi = "10.18653/v1/2021.emnlp-main.619",
    pages = "7856--7870",
}

@inproceedings{wolf-etal-2020-transformers,
    title = "Transformers: State-of-the-Art Natural Language Processing",
    author = "Wolf, Thomas  and
      Debut, Lysandre  and
      Sanh, Victor  and
      Chaumond, Julien  and
      Delangue, Clement  and
      Moi, Anthony  and
      Cistac, Pierric  and
      Rault, Tim  and
      Louf, Remi  and
      Funtowicz, Morgan  and
      Davison, Joe  and
      Shleifer, Sam  and
      von Platen, Patrick  and
      Ma, Clara  and
      Jernite, Yacine  and
      Plu, Julien  and
      Xu, Canwen  and
      Le Scao, Teven  and
      Gugger, Sylvain  and
      Drame, Mariama  and
      Lhoest, Quentin  and
      Rush, Alexander",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: System Demonstrations",
    month = oct,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-demos.6",
    doi = "10.18653/v1/2020.emnlp-demos.6",
    pages = "38--45",
    abstract = "Recent progress in natural language processing has been driven by advances in both model architecture and model pretraining. Transformer architectures have facilitated building higher-capacity models and pretraining has made it possible to effectively utilize this capacity for a wide variety of tasks. Transformers is an open-source library with the goal of opening up these advances to the wider machine learning community. The library consists of carefully engineered state-of-the art Transformer architectures under a unified API. Backing this library is a curated collection of pretrained models made by and available for the community. Transformers is designed to be extensible by researchers, simple for practitioners, and fast and robust in industrial deployments. The library is available at https://github.com/huggingface/transformers.",
}

